CoMM: A Coherent Interleaved Image-Text Dataset for Multimodal Understanding and Generation

Interleaved image-text generation has emerged as a crucial multimodal task, aiming at creating sequences of interleaved visual and textual content given a query. Despite notable advancements in recent multimodal large language models (MLLMs), generating integrated image-text sequences that exhibit narrative coherence and entity and style consistency remains challenging due to poor training data quality. To address this gap, we introduce CoMM, a high-quality Coherent interleaved image-text MultiModal dataset designed to enhance the coherence, consistency, and alignment of generated multimodal content. Initially, CoMM harnesses raw data from diverse sources, focusing on instructional content and visual storytelling, establishing a foundation for coherent and consistent content. To further refine the data quality, we devise a multi-perspective filter strategy that leverages advanced pre-trained models to ensure the development of sentences, consistency of inserted images, and semantic alignment between them. Various quality evaluation metrics are designed to prove the high quality of the filtered dataset. Meanwhile, extensive few-shot experiments on various downstream tasks demonstrate CoMM's effectiveness in significantly enhancing the in-context learning capabilities of MLLMs. Moreover, we propose four new tasks to evaluate MLLMs' interleaved generation abilities, supported by a comprehensive evaluation framework. We believe CoMM opens a new avenue for advanced MLLMs with superior multimodal in-context learning and understanding ability.

==> tables/task1_results.tex <==
\begin{table}[t]
% \tabcolsep=0.8mm
\centering
\caption{Performance comparison among MiniGPT-5~\cite{zheng2023minigpt}, SEED-Llama~\cite{ge2023making}, and Emu2~\cite{sun2023emu} on Image-to-Text Sequence Generation task and Text-to-Image Sequence Generation task. ``M.S.'' and ``R.S. '' mean METEOR~\cite{banerjee2005meteor} and ROUGE\_L~\cite{lin2004rouge} on each step evaluation and ``M.W.'' and ``R.W.'' denote METEOR~\cite{banerjee2005meteor} and ROUGE\_L~\cite{lin2004rouge} on whole docs evaluation. }
\small
\begin{tabular}{cc|cccc|cccc}
% \noalign{\hrule height 1.5pt}
\toprule
 \multirow{2}{*}{Methods} & \multirow{2}{*}{Size} & \multicolumn{4}{c|}{I2T Sequence Generation (Task1)} & \multicolumn{4}{c}{T2I Sequence Generation (Task2)} \\
        &  & M.S. &      R.S.     &     M.W.    &     R.W.  &   FID $\downarrow$ &  IS &  SSIM &  PSNR \\
\midrule
 MiniGPT-5~\cite{zheng2023minigpt} & 7B & 4.60 & 8.64 & 9.10  & 10.67  & 49.76 & 6.74 & 22.66 & 7.57 \\
 SEED-Llama~\cite{ge2023making} & 8B &  2.29 & 6.34 & 4.20  & 7.33  &  57.96 & 8.40 & 20.53 & 7.87 \\
 SEED-Llama~\cite{ge2023making} & 14B &  3.16 & 8.12 & 5.71  & 8.17  &  66.23 & 11.06 & 20.83 & 8.12 \\
 Emu2~\cite{sun2023generative}& 33B & 3.65 & 8.41 & 7.43 & 8.62  & 60.45 & 6.34 & 20.96 & 7.91 \\

\bottomrule
\end{tabular}
\label{table:task1_reuslts}
\end{table}




==> tables/task2_results.tex <==
% \begin{table}[t]
% \tabcolsep=0.9mm
% \centering
% \caption{Performance comparison among MiniGPT-5~\cite{zheng2023minigpt}, SEED-Llama~\cite{ge2023making}, and Emu2~\cite{sun2023emu} on Text-to-Image Sequence Generation task. }
% \small
% \begin{tabular}{cc|ccccccccc}
% % \noalign{\hrule height 1.5pt}
% \toprule
% Methods & Size &  FID $\downarrow$ &  IS &  SSIM &  PSNR &  Style  &   Entity  &    Trend &  ImgQ & T2I\\
% \midrule
%  MiniGPT-5~\cite{zheng2023minigpt} & 7B &  &  &   &    \\
%  SEED-Llama~\cite{ge2023making} & 8B &  77.37 & 8.32  & 20.07 & 7.84 &  \\
%  SEED-Llama~\cite{ge2023making} & 14B & 77.03 & 8.76  & 20.85 & 8.06  \\
%  Emu2~\cite{sun2023generative}& 33B & 44.42 & 6.26 & 24.46 & 7.78  \\

% \bottomrule
% \end{tabular}
% \label{table:task2_reuslts}
% \end{table}

==> tables/task3_results.tex <==
\begin{table}[t]
    \tabcolsep=0.9mm
    \centering
    \caption{Performance comparison among MiniGPT-5~\cite{zheng2023minigpt}, SEED-Llama~\cite{ge2023making}, and Emu2~\cite{sun2023generative} on Question-based Interleaved Image-Text Generation. ``CPL.'' refers to Completeness, ``ImgQ'' denotes Image Quality, and ``TFI'' means Text Fidelity to Images.}
    \small
    \begin{tabular}{cc|cccccc|cccccc}
    % \noalign{\hrule height 1.5pt}
    \toprule
    \multirow{2}{*}{Methods} & \multirow{2}{*}{Size} & \multicolumn{6}{c|}{Continuation Generation (Task3)} &  \multicolumn{6}{c}{ Question-based  Generation (Task4)}  \\
     &  &  Style  &   Entity  &    Trend & CPL. & ImgQ & TFI &  Style  &   Entity  &    Trend & CPL. & ImgQ & TFI \\
    \midrule
     MiniGPT-5~\cite{zheng2023minigpt} & 7B & 5.58 & 5.21 & 5.24  & 6.33  & 6.36 & 2.56  &  5.65 & 5.20 & 5.25 & 5.81 & 6.15 & \textbf{2.71}   \\
     SEED-Llama~\cite{ge2023making} & 8B & 6.28 & 5.84 & 5.72  & 6.28 & 6.55 & 2.92  & 7.55 & 6.81 & 6.15  & 5.13 &6.36 & 1.46 \\
     SEED-Llama~\cite{ge2023making} & 14B & 6.68 & 6.22 & 6.13 & 6.66  & 6.67 & \textbf{3.23} & 7.51  & 6.61 & 6.30 & 6.13 & 6.66  & 2.50 \\
     Emu2~\cite{sun2023generative}& 33B & \textbf{8.22} & \textbf{7.99} & \textbf{7.97}  & \textbf{8.49} & \textbf{8.62} & 2.42 & \textbf{8.41}  & \textbf{7.56} & \textbf{7.63} & \textbf{7.54} & \textbf{7.59} & 2.02  \\
    
    \bottomrule
    \end{tabular}
    \label{table:task4_reuslts}
\end{table}

% \begin{table}[t]
% \begin{minipage}[b]{0.48\linewidth}
%     \tabcolsep=0.5mm
%     \centering
%     \caption{Performance comparison among MiniGPT-5~\cite{zheng2023minigpt}, SEED-Llama~\cite{ge2023making}, and Emu2~\cite{sun2023emu} on Interleaved Image-Text content continuation task. }
%     \begin{tabular}{cc|cccc}
%     % \noalign{\hrule height 1.5pt}
%     \toprule
%     Methods & Size &  Met.1  &   Met.2  &  Met.3   &  Ave. \\
%     \midrule
%      MiniGPT-5~\cite{zheng2023minigpt} & 7B &  &  &   &    \\
%      SEED-Llama~\cite{ge2023making} & 8B &  &  &   &    \\
%      SEED-Llama~\cite{ge2023making} & 14B &  &  &   &    \\
%      Emu2~\cite{sun2023emu}& 33B &  &  &   &    \\
    
%     \bottomrule
%     \end{tabular}
%     \label{table:task3_reuslts}
% \end{minipage}
% \hspace{2mm}
% \begin{minipage}[b]{0.48\linewidth}
%     \tabcolsep=0.5mm
%     \centering
%     \caption{Performance comparison among MiniGPT-5~\cite{zheng2023minigpt}, SEED-Llama~\cite{ge2023making}, and Emu2~\cite{sun2023emu} on Question-based Interleaved Image-Text Generation. }
%     \begin{tabular}{cc|cccc}
%     % \noalign{\hrule height 1.5pt}
%     \toprule
%     Methods & Size &  Met.1  &   Met.2  &  Met.3   &  Ave. \\
%     \midrule
%      MiniGPT-5~\cite{zheng2023minigpt} & 7B &  &  &   &    \\
%      SEED-Llama~\cite{ge2023making} & 8B &  &  &   &    \\
%      SEED-Llama~\cite{ge2023making} & 14B &  &  &   &    \\
%      Emu2~\cite{sun2023emu}& 33B &  &  &   &    \\
    
%     \bottomrule
%     \end{tabular}
%     \label{table:task3_reuslts}
% \end{minipage}
% \end{table}




